Type-Based Verification of Delegated Control in Hybrid~Systems (Full Version)

We present a post-region-based verification system for distributed hybrid systems modeled with Hybrid Active Objects. The post-region of a class method is the region of the state space where a physical process must be proven safe to ensure some object invariant. Prior systems computed the post-region locally to a single object and could only verify systems where each object ensures its own safety, or relied on specific, non-modular communication patterns. The system presented here uses a type-and-effect system to structure the interactions between objects and computes post-regions globally, but verifies them locally. Furthermore, we are able to handle systems with delegated control: the object and method that shape the post-region change over time. We exemplify our approach with a model of a cloud-based hybrid system.

==> _core.tex <==


\subsection{Goal}

The goal of this type system is to ensure that on every objects,
 the time laps between two calls of the same method is bound by a number specified by the user,
 and also that the max number of concurrent calls is also bound.

Over the time, several approaches were discussed, and currently, the design choice we have are as follow:
\begin{itemize}
\item  every {\em capability} is the responsibility of exactly one method at every point in time
\item {\em capabilities} are garbage collected when they are not reachable anymore.
\end{itemize}
Of course, when I say {\em capability}, I mean every method of every object that must be called periodically.

These design choices give rise to a system in which we ensure for every capability tracked in a method's body, that it is the responsibility of some method, and if that method is the current one, then we need to keep track of lapsed time to ensure that that capability is called as often as necessary.

This principle is quite simple (keeping track of capabilities) but is based on two complex models:
\begin{itemize}
\item {\em counting time}. In ABS, time passing is counted with rational numbers, and so, capability requirement could be expressed in any decidable logic over rational number.
\item {\em deciding termination}. Since in ABS it is possible to wait for a method to finish, we need a way to estimate how much time passed during this waiting and which other methods completed during this elapsed time.
\end{itemize}
Hence, any analysis we may propose here must be based on a logic over rational numbers
 and some analysis for method termination.
Since such analysis does not depend on the internals of these models, we design in the following such an analysis that is parametric.

\subsection{Global Analysis}

Our type system is parametric on two external analysis that give information about time passing and object identity in the program.


\begin{definition}
We suppose that every node of the AST has a unique identity.
We write $\mathcal{I}$ the set of all these ids.
\end{definition}


Notion of logic of time.
Maybe needs some refinements.
\begin{definition}
A {\em Rational Time Logic} (RTL) is a tuple $(E,P,\vdash,\infty)$ where:
 $E$ is an {\em expression language} such that if $e_1,e_2\in E$, then $e_1-e_2\in E$;
 $P$ is a {\em proposition language} such that if $e_1,e_2\in E$, then $e_1\leq e_2\in P$;
 $\vdash$ is a subset of $P$, stating which propositions are valid (we write $\vdash P$ for $p\in\vdash$);
 $\infty\in E$ is such that for all $e\in E,\, \vdash e\leq \infty$ and if $(\infty\leq e)\not\in\vdash$, $\vdash \infty\leq\infty-e$ holds.
\end{definition}

Notion of time oracle: gives time passing and effect on future identities.
Need to give a more precise definition of correctness, but should be ok for now.
\begin{definition}
Given a RTL $(E,P,\vdash,\infty)$, a {\em Time Oracle} (TO) is a pair $(\mathcal{F}, C,E)$ where:
 $\mathcal{F}$ is a set of future identity;
 $C$ is a partial injective function from $\mathcal{I}$ to $\mathcal{F}$ (for process creation);
 $E$ is a partial function from $\mathcal{I}$ to pairs $(E, \{f_i,E_i\}_{i\in I})$ that give the time the AST node took to compute,
  and the set of all future that are known to have finished during this time period and since when they might have finished;
 and $\dom(C)\cap\dom(E)=\emptyset$.

A TO is {\em correct} w.r.t. a program $P$ iff for all traces of that program:
 there is a mapping $m_f$ from futures in the trace of the program to $\mathcal{F}$
  such that all futures $f$ are indeed created by statement $i$ with $m_f(f)=C(i)$;
 all processes are concluded in the time frame stated by the oracle (between the sure end $E$ minus $E_i$ and the sure end $E$).
\end{definition}

Notion of Alias analysis: gives the object identity for every expression
\begin{definition}
An {\em alias analysis} (AA) is a pair $(\mathcal{O},\mathit{Id})$ such that:
  $\mathit{Id}$ is a partial mapping from $\mathcal{I}$ to $\mathcal{O}$.

A AA is {\em satisfactory} iff its domain contains all nodes that are typed with a capable type.

A AA is {\em correct} w.r.t. a program $P$ iff for all traces of that program:
 if two expressions $i_1,i_2$ in the domain of $\mathit{Id}$ respectively evaluates to $o$ and $o'$ then we have
 $(o=o')$ iff $(\mathit{Id}(i_1)=\mathit{Id}(i_2))$.
\end{definition}

\begin{definition}
if we do not want to ensure lower bound for method call, we only need one implication in the AA correction:
$(\mathit{Id}(i_1)=\mathit{Id}(i_2))$ implies $(o=o')$.
\end{definition}

\subsection{Global Data}

We need a table of which types are capable, and which methods take responsibility of which parameters

\subsection{Rules}


\begin{remark}
The oracle $O$ must state which futures are sure to be completed, and how much time at most lapsed since they completed (to ensure that at every point in time, only one future is responsible of a capability)
\end{remark}

\begin{remark}
Since we consider that once a controlled object is created, it must be controlled forever, the main block cannot finish.
We model that fact by removing all information from the type effect whenever that entry is controlled by a future that never finishes.
With this encoding, a correct program has empty effects (all the controlled objects are managed by infinitely computing processes).
\end{remark}

\begin{remark}
Even with alias analysis, it is impossible without a dedicated analysis to check if a controlled object has multiple concurrent controllers if it is shared in an object field.
Indeed, the object can be created somewhere, and the field can be set somewhere else, and a controller method can be called somewhere else entirely again. To capture this, we need a fancy may-happen-in-parallel analysis that also captures aliases and state. Technically, this could be done with the deadline analysis (which gives a sort of may-happen-in-parallel analysis), but then the check is global -- not syntax-driven -- on that analysis: is there two controlling methods running on the same field at the same time.

The second problem occurring for fields is how to ensure that they managed correctly (i.e., their methods are called regularly enough). Again, this can be ensured by the MHP analysis if it can state that the delay between two controlling calls on every field is short enough. How to do this is a bit unclear, so, with the other difficulties mentioned before (the need of a alias-checking MHP analysis), and the lack of usecases, I would forbid in a first time controlled objects as fields (or forbidding to call controlling methods on controlled fields).
\end{remark}

\begin{rules}
% rule prgm
\entry{
  \text{\it gettable}(\xabs{Prgm}) = \ctable\and
  \xabs{Prgm} = \xabs{CD}_1\ \dots\ \xabs{CD}_n\ \{s\} \\
  \ctable,\cdeadline,\calias\typep \xabs{CD}_i \and
  \ctable,\cdeadline,\calias,\emptyset,\emptyset \typep \xabs{s} \typep \emptyset
}{
  \cdeadline,\calias\typep \text{\abs{Prgm}}
}
% rule for entry deletion
\entry{
  \ctable,\cdeadline,\calias,\Gamma, m' \typep \text{\abs{s}} \typed m\uplus[o.\text{\abs{m}}\mapsto (f,e)]\\
  \cdeadline.\text{\it is\_infinite}(f)
}{
  \ctable,\cdeadline,\calias,\Gamma, m' \typep \text{\abs{s}} \typed m
}
% rule for classes
\and
\entry{
\xabs{T}_i\not\in\dom(\ctable.\text{\it controlled})\\
\ctable,\cdeadline,\calias,\xabs{C},[\xabs{this}.x_i\mapsto \xabs{T}_i]\typep \xabs{Mt}_i
}{
 \ctable,\cdeadline,\calias\typep \xabs{class C}(\xabs{T}_1\ x_1\ \dots\ \xabs{T}_l\ x_l) \{\xabs{T}_{l+1}\ x_{l+1}\ \dots\ \xabs{T}_m\ x_m\ \xabs{Phys}\ \xabs{Mt}_1\ \dots\ \xabs{Mt}_n\}
}
% rule for methods
\and
\entry{
  \ctable,\cdeadline,\calias,\Gamma[x_i\mapsto \xabs{T}_i],[c\mapsto \ctable.\text{\it controlling}(\xabs{C.m})(c)[\text{\rm begin}]\mid c\in\dom(\ctable.\text{\it controlling}(\xabs{C.m}))]\typep \xabs{s}\typed m\\
  \dom(m)=\dom(\ctable.\text{\it controlling}(\xabs{C.m}))\\
  \forall c\in\dom(m),\, m(c)\geq \ctable.\text{\it controlling}(\xabs{C.m})(c)[\text{\rm end}]
}{
  \ctable,\cdeadline,\calias,\xabs{C},\Gamma\typep \xabs{T m}(\xabs{T}_1\ x_1\ \dots\ \xabs{T}_n\ x_n)\{\xabs{s; return e;}\}
}
% rule for wait
\and
\entry{
\xabs{s}=\wait(sync) \lor \xabs{s}=(x = y.\xabs{get}) \lor \xabs{s}=\xabs{duration(s)}\\
  \cdeadline(s)=(
    l, % the maximal time that passed during this await statement
    \{(f_k,l_k')\sht k\in K\} % gives for every future that is known to have finished, how much time at most passed since it finished
  )\text{ with $K\subseteq J$}
  \\
  % compute the new capability deadlines
  m = [c_i\mapsto (\xabs{this}, l_i-l)]_{i\in I}+[c_k\mapsto (\xabs{this},l_k-l-l_k')]_{k\in K}
  \\
  % check that they are all valid
  \forall (c,(\text{\abs{this}}, v))\in m,\,v\geq 0
}{
  \ctable, \cdeadline,\calias, \Gamma,[c_i\mapsto (\text{\abs{this}}, l_i)]_{i\in I}+[c_j\mapsto (f_j, l_j)]_{j\in J}
  \vdash \xabs{s} \typed m+[c_j\mapsto (f_j, l_j)]_{j\in J\setminus K}
}
% rule for method call
\and
\entry{
  \calias(\xabs{e}_i)=x_i\\
  \calias(\xabs{e$_0$!m(e$_1$, $\dots$, e$_n$)})=f\\
%   \calias(\lstinline[mathescape=true]|e$_0$!m(e$_1$, $blabla$, e$_n$)|)=f\\
  \Gamma(x_i)=\xabs(T)_i\\
  \ctable.\text{\it controlling}(\xabs{T}_0)=[i\mapsto \{(\xabs{m}_i^j, e_{i,1}^j, e_{i,2}^j)\mid j\in J_i\}]_{0\leq i}^n\\
  \forall i,j,k,\,x_i.\xabs{m}_i^j=x_k.\xabs{m}_k\Rightarrow e_k - e_{i,1}^j \geq 0\\
%   I'=[1..n]\cap\{i\mid x_i\in\dom(\Gamma)\land\Gamma(x_i)\in\dom(\ctable.\text{\it controlled})\}\\
%  \ctable.\text{\it controlled}(\xabs(T.m))
m'=m[x_0.\xabs{m}\mapsto\ctable.\text{\it controlled}(\xabs{T$_0$.m})] + [x_i.\xabs{m}_i^j\mapsto(f, e_{i,2}^j)]_{i,j}
}{
\ctable,\cdeadline,\calias,\Gamma, m+[x_k.\xabs{m}_k\mapsto (\xabs{this},e_k)]_{k\in K}\typep \xabs{T $x$ = e$_0$!m(e$_1$, $\dots$, e$_n$)}\typed \Gamma[x:f] \mid m'
}
% rule for object creation/declaration

\end{rules}


\begin{remark}
I need to normalize the API of the different analysis and use the equality decision of the alias analysis,
instead of replacing names with identities.

So, to simplify things, I should have:
\begin{itemize}
\item $\Gamma$ that stores the type of variables, without considering identities
\item $m$ (and {\it controlling}) is equivalent to adding entries with $\infty$ so we can remove the typing rule, and have only one rule for method call
\end{itemize}
\end{remark}


\subsection{On Typing precision}

As it is designed, the type system ensures that every variable with a sensitive type has a controller that manages it correctly.
This design can be refined in several ways.

\paragraph{Several Controllers.} the mapping used to check if a variable is controlled only associates one future information per variable, which means that calling two concurrent controller on the same variable is not validated by the type system.

If such a flexibility is desired, it is possible for the mapping to associates a variable to a set of future information.
That set is correct as long as there is one future information with a positive or null deadline, and upon the end of a future, the \abs{this} future is updated with the deadline associated to it.

\paragraph{Less redundant checks.} it is possible that two variables actually refer to the same object. This means that in our setting, we enforce in some case that a controlled object has several concurrent controller.

It is possible to have a more flexible analysis by using an additional alias analysis $\mathcal{A}$, that analyses the mapping and unifies the entries corresponding to the same object (e.g., $\mathcal{A}(m)$ takes the mapping $m$ and unifies the entries of the variables $\mathcal{A}$ knows for sure to be equal). This extension does not require a perfect alias analysis.

\paragraph{Unique Controllers.} In some other case, for instance when we want to ensure that the time delay between two calls to a sensitive method has a lower bound, we may need to enforce the fact that such methods only have one controller at all time.

This property requires to adapt our type system to become an ownership one, possibly using an alias analysis that can perfectly detect the identity of controlled object (possibly through the use of some restriction on the language constructions). In that case the analysis $\mathcal{A}$ must ensure that the mapping $\mathcal{A}(m)$ (we still consider that two variables can refer the same object) only give one future information per entry.



\subsection{Language Syntax}
\begin{syntax}
\entry s = 0 \bnfor \nu x; s \bnfor \nu f=x.m(\vect{e}) \bnfor \sync{f};s \bnfor \wait(e_n);s [{}]
\entry e = e_n \bnfor x [{}]
\entry e_n = u \bnfor k \bnfor e_n + e_n [{}]
%
\entry P = m_1(p_1)=s_1 \dots m_n(p_n)=s_n\ \texttt{main}(x,u)=s [{}]
\end{syntax}




\subsection{Type Syntax}
\begin{syntax}
\entry l = {(k;k;k)[k]} [{}]
\entry \tau = {[m_i\rightarrow l_i]_{1\leq i\leq n}} [{}]
\end{syntax}
A type $\tau$ gives information on the usage of every methods $m_i$ in the program.
The usage $l=(k_i;k_r;k_e)[k_u]$ contains four information:
 $k_i$ is the amount of time before this method is called;
 $k_r$ is the maximum amount of time between two consecutive call of this method;
 $k_e$ is the time passed after the last call to the method;
 and $k$ is the maximal number of concurrent calls of that method.
 

\subsection{Type System}

The idea is to annotate every method arguments (that is not a number) and every object creation with a type $\tau$ informing on the usage of every methods (we will see in a second time how to deal with partial declarations).

\begin{center}\bf
!!!! WARNING !!!!:\\
 do we want to allow for some method calls not to be synchronized\\(this duplicates the types, c.f. work on deadlock).
\end{center}

So, the type system for linear time is simple: for every method usage specification, we remove the elapsed time from $k_i$,
 reset it with $k_r$ when the method is called, and at the end of the method we just have to check that $(k_r-k_i)\leq k_e$.
Of course, this works when we consider that every methods is called at least one.

\bigskip


The interesting part is non-linear time, i.e., when we have future (that we consider always synchronized for now).
For every future, we can do like it is done in the time analysis: we store the information for each future like it started at the beginning of the current method, and at synchronization point, we check the merge of the two types.
So, when computing the type of the future, we need to check that it validates the specification of every parameter













\newpage

VERSION WITHOUT P


\begin{rules}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% method declaration
\entry{
  \getanncontrolling(\xabs{C.m})=[\xabs{x}_i.\xabs{m}_j\mapsto[t_j, t_j']]_{i\in I,j\in J_i}\and
  \forall i\in I,\forall j\in J_i,\, \getanncontrolled(\xabs{T}_i.\xabs{m}_j) \geq t_j \\{}
  [\xabs{x}_i.\xabs{m}_j:t_j]_{i\in I,j\in J_i},\emptyset\typep \xabs{s} \typed [\xabs{x}_i.\xabs{m}_j:t_j'']_{i\in I',j\in J_i'},\emptyset\\
  I'\subseteq I\and \forall i\in I',\,J_i'\subseteq J_i\land \forall j\in J_i,\, t_j'\geq t_j''
}{\xabs{C}\typep\xabs{T m(T$_1$ y$_1$, $\dots$, T$_n$ y$_n$) \{s;return e;\}}}
\end{rules}


\begin{rules}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% can remove \infty from effect
\entry{
  \Gamma_l,\Gamma_d\typep \xabs{s}\typed [\coreid_i\mapsto t_i]\uplus[\coreid\mapsto t],\Gamma_d' \and t\geq\infty
 }{\Gamma_l,\Gamma_d\typep \xabs{s}\typed [\coreid_i\mapsto t_i],\Gamma_d'}
\end{rules}
\begin{rules}
\entry{
  \Gamma_l,\Gamma_d\typep \xabs{s}\typed \Gamma_l',[\coreid_i\mapsto (\mathit{fid}_i, t_{i,1}, t_{i,2}, t_{i,3})]\uplus[\coreid\mapsto (\mathit{fid}, t_1, t_2, t_3)] \and t_1\geq\infty
 }{\Gamma_l,\Gamma_d\typep \xabs{s}\typed \Gamma_l',[\coreid_i\mapsto (\mathit{fid}_i, t_{i,1}, t_{i,2}, t_{i,3})]}
\end{rules}



\begin{rules}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% statements
\entry{
  \Gamma_l,\Gamma_d\typep \xabs{s}_1\typed \Gamma_{l,1},\Gamma_d'\\
  \Gamma_l,\Gamma_d\typep \xabs{s}_2\typed \Gamma_{l,2},\Gamma_d'\\
  \dom(\Gamma_{l,1})=\dom(\Gamma_{l,2})\\
  \Gamma_l'=[\coreid\mapsto\min(\Gamma_{l,1}(\coreid), \Gamma_{l,2}(\coreid))]_{\coreid\in\dom(\Gamma_{l,1})}
}{\Gamma_l,\Gamma_d\typep \xabs{if(e) \{ s$_1$\} else \{ s$_2$ \}}\typed\Gamma_l',\Gamma_d'}
\end{rules}
\begin{rules}
\entry{
  \Gamma_l,\Gamma_d\typep \xabs{s}_1\typed \Gamma_l',\Gamma_d'\\
  \Gamma_l',\Gamma_d'\typep \xabs{s}_2\typed \Gamma_l'',\Gamma_d''
}{\Gamma_l,\Gamma_d\typep \xabs{s$_1$ ; s$_2$}\typed\Gamma_l'',\Gamma_d''}
\end{rules}
\begin{rules}
\entry{
  \Gamma_l,\Gamma_d\typep^{\mathit{t}} \xabs{await g}\typed \Gamma_l',\Gamma_d'
}{\Gamma_l,\Gamma_d\typep \xabs{await g}\typed\Gamma_l',\Gamma_d'}
\end{rules}
\begin{rules}
\entry{
  \Gamma_l,\Gamma_d\typep \xabs{rhs}\typed [\xabs{m}_i\mapsto t_i]_{i\in I},\Gamma_l',\Gamma_d'\\
  \Gamma_l''=\Gamma_l'\uplus[\xabs{x.m}_i\mapsto t_i]_{i\in I}\\
  \Gamma_l'',\Gamma_d'\typep^{\mathit{t}} \xabs{T x = rhs}\typed \Gamma_l''',\Gamma_d''
}{\Gamma_l,\Gamma_d\typep \xabs{T x = rhs}\typed\Gamma_l''',\Gamma_d''}
\end{rules}
\begin{rules}
\entry{
  \Gamma_l,\Gamma_d\typep^{\mathit{t}} \xabs{duration(e)}\typed \Gamma_l',\Gamma_d'
}{\Gamma_l,\Gamma_d\typep \xabs{duration(e)}\typed\Gamma_l',\Gamma_d'}
\end{rules}


\begin{rules}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% statement that take time
\entry{
\TA(\xabs{s})=[t_{\min},t_{\max}]\\
% update
\Gamma_{l,1}=[\coreid\mapsto\Gamma_l(\coreid) - t_{\max}]_{\coreid\in\dom(\Gamma_l)}\\
% split delegated
C=\{\coreid\mid\coreid\in I\land t_\coreid^2<t_{\min}\}\\
%
\Gamma_d'=[\coreid\mapsto(\mathit{fid}, t_\coreid^1-t_{\max}, t_\coreid^2-t_{\min}, t_\coreid^3)]_{\coreid\in \dom(\Gamma_d)\setminus C}\\
\Gamma_{l,2}=[\coreid\mapsto t_\coreid^3 + (t_{\max}-t_\coreid^1)]_{\coreid\in C}\\
% combine and check
\Gamma_l'=\Gamma_{l,1}\uplus \Gamma_{l,2}\and
\forall \coreid\in\dom(\Gamma_l'),\,\Gamma_l'(\coreid) \geq 0
}{\Gamma_l,[\coreid\mapsto(\mathit{fid}, t_\coreid^1, t_\coreid^2, t_\coreid^3]_{\coreid\in I}\typep^{\mathit{t}}\xabs{s}\typed \Gamma_l',\Gamma_d'}
\end{rules}


\begin{rules}
\axiom{\Gamma_l,\Gamma_d\typep \xabs{e}\typed \emptyset, \Gamma_l,\Gamma_d}
\end{rules}
\begin{rules}
\entry{
  M = \{\xabs{m}\sht \xabs{C.m}\in\dom(\getanncontrolled)\}\\
  S=[\xabs{m}\mapsto \getanncontrolled(\xabs{C.m})]_{\xabs{m}\in M}
}{\Gamma_l,\Gamma_d\typep \xabs{new C(e$_1$,$\dots$,e$_n$)} \typed S, \Gamma_l,\Gamma_d}
\end{rules}
\begin{rules}
\axiom{\Gamma_l,\Gamma_d\typep \xabs{e.get}\typed \emptyset, \Gamma_l,\Gamma_d}
\end{rules}
\begin{rules}
\entry{
  \forall 1\leq i\leq n,\,\mathit{type}(\xabs{e}_i)=\xabs{T}_i \and % type each expression
  \getanncontrolling(\xabs{T$_1$.m})=[\xabs{x}_i.\xabs{m}_j\mapsto[t_j, t_j']]_{i\in I,j\in J_i}\\
  % update \Gamma with the call
  \Gamma_l'\uplus[\xabs{e}_i.\xabs{m}_j\mapsto t_j'']_{i\in I,j\in J_i}=\left\{\begin{array}{ll}
  \Gamma_l[\xabs{e}_1.\xabs{m}\mapsto\getanncontrolled(\xabs{T$_1$.m})] & \text{if $\xabs{e}_1.\xabs{m}\in\dom(\Gamma_l)$}\\
  \Gamma_l & \text{else}
  \end{array}\right.\\
  % update \Gamma with the control delegation
  \forall i\in I,\forall j\in J_i,\, t_j'' \geq t_j \and
  \TA(\xabs{T$_1$.m})=[t_1,t_2] \and \mathit{fid}\ \text{\rm fresh}
}{\Gamma_l,\Gamma_d\typep \xabs{e$_1$!m(e$_2$,$\dots$,e$_n$)} \typed
  \emptyset, \Gamma_l'',\Gamma_d[\xabs{e}_i.\xabs{m}_j\mapsto (\mathit{fid}, t_1, t_2, t_j')]_{i\in I,j\in J_i}}
\end{rules}







\newpage


\newpage


To illustrate our type system, we informally describe some of its typing rules.
The rules are given in Figure~\ref{fig:ts-subset}.

Every node of the AST is tagged, and we have getters on the nodes.
$\tapreds$, $\getanncontrolling$ and $\getanncontrolled$, $\TA{\text{\sf Prgm}}$, $\cfispositive$, $\cfisinfty$, $\mathit{type}$
\begin{figure}
\begin{rules}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% method declaration
\entry{
  \getanncontrolling(\xabs{C.m})=[\xabs{x}_i.\xabs{m}_j\mapsto[t_{i,j}, t_{i,j}']]_{i\in I\subseteq[1..n], j\in J_i}\\ % get controlling annotation from the method
  \getanncontrolled(\xabs{T}_i.\xabs{m}_j)=t_{i,j}''\\ % get controlled annotation from the method
  %\forall 1\leq i\leq n,\, \forall \xabs{m}\ \text{method of}\ \xabs{T}_j,\, % all ceid that need control are controlled
  %  ((\exists j\in J_i,\,\xabs{m}=\xabs{m}_j) \lor (\xabs{T}_i.\xabs{m}\not\in\dom(\getanncontrolled))\\
  \forall \xabs{x}_i.\xabs{m}_j,\, \cfispositive(t_{i,j}'' - t_{i,j}) \\ % check that the initial delay is ok
  % type the method for all its possible execution context
  c=\{P\sht P\in\tapreds\land\exists \xabs{e}_1,\dots,\xabs{e}_n,\,P(\xabs{C.m}, \xabs{e}_1,\dots,\xabs{e}_n)\}\\
  \forall P\in c,\left(\begin{array}{c}
  [\xabs{x}_i.\xabs{m}_j:t_{i,j}]_{i\in I\subseteq[1..n], j\in J_i},\emptyset\typep_P \xabs{s} \typed 
    [\xabs{x}_i.\xabs{m}_j:t_{i,j}^P]_{i_P\in I^P, j_P\in J_i^P},\emptyset\\ I^P\subseteq I \and J_i^P\subseteq J_i\\
  \forall \xabs{x}_i.\xabs{m}_j,\, \cfispositive(t_{i,j}' - (t_{i,j}''-t_{i,j}^P)) % check that the final delay is ok for all possible execution
  \end{array}\right)
}{\xabs{C}\typep\xabs{T m(T$_1$ x$_1$, $\dots$, T$_n$ x$_n$) \{s;return e;\}}}
\and
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% can remove \infty from effect
\entry{
  \Gamma_l,\Gamma_d\typep_P \xabs{s}\typed [\coreid_i\mapsto t_i]\uplus[\coreid\mapsto t],\Gamma_d' \and \cfisinfty(t)
 }{\Gamma_l,\Gamma_d\typep_P \xabs{s}\typed [\coreid_i\mapsto t_i],\Gamma_d'}
 \and
\entry{
  \Gamma_l,\Gamma_d\typep_P \xabs{s}\typed \Gamma_l',[\coreid_i\mapsto (\mathit{fid}_i, t_{i,1}, t_{i,2}, t_{i,3})]\uplus[\coreid\mapsto (\mathit{fid}, t_1, t_2, t_3)] \and \cfisinfty(t_1)
 }{\Gamma_l,\Gamma_d\typep_P \xabs{s}\typed \Gamma_l',[\coreid_i\mapsto (\mathit{fid}_i, t_{i,1}, t_{i,2}, t_{i,3})]}
 \and
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% statements
\entry{
  \Gamma_l,\Gamma_d\typep_P \xabs{s}_1\typed \Gamma_{l,1},\Gamma_d'\\
  \Gamma_l,\Gamma_d\typep_P \xabs{s}_2\typed \Gamma_{l,2},\Gamma_d'\\
  \dom(\Gamma_{l,1})=\dom(\Gamma_{l,2})\\
  \Gamma_l'=[\coreid\mapsto\min(\Gamma_{l,1}(\coreid), \Gamma_{l,2}(\coreid))]_{\coreid\in\dom(\Gamma_{l,1})}
}{\Gamma_l,\Gamma_d\typep_P \xabs{if(e) \{ s$_1$\} else \{ s$_2$ \}}\typed\Gamma_l',\Gamma_d'}
\and
%
\entry{
  \Gamma_l,\Gamma_d\typep_P \xabs{s}_1\typed \Gamma_l',\Gamma_d'\\
  \Gamma_l',\Gamma_d'\typep_P \xabs{s}_2\typed \Gamma_l'',\Gamma_d''
}{\Gamma_l,\Gamma_d\typep_P \xabs{s$_1$ ; s$_2$}\typed\Gamma_l'',\Gamma_d''}
\and
\entry{
  \Gamma_l,\Gamma_d\typep_P^{\mathit{t}} \xabs{await g}\typed \Gamma_l',\Gamma_d'
}{\Gamma_l,\Gamma_d\typep_P \xabs{await g}\typed\Gamma_l',\Gamma_d'}
\and
\entry{
  \Gamma_l,\Gamma_d\typep_P \xabs{rhs}\typed [\xabs{m}_i\mapsto t_i]_{i\in I},\Gamma_l',\Gamma_d'\\
  \Gamma_l''=\Gamma_l'\uplus[\xabs{x.m}_i\mapsto t_i]_{i\in I}\\
  \Gamma_l'',\Gamma_d'\typep_P^{\mathit{t}} \xabs{T x = rhs}\typed \Gamma_l''',\Gamma_d''
}{\Gamma_l,\Gamma_d\typep_P \xabs{T x = rhs}\typed\Gamma_l''',\Gamma_d''}
\and
\entry{
  \Gamma_l,\Gamma_d\typep_P^{\mathit{t}} \xabs{duration(e)}\typed \Gamma_l',\Gamma_d'
}{\Gamma_l,\Gamma_d\typep_P \xabs{duration(e)}\typed\Gamma_l',\Gamma_d'}
\and
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% statement that take time
\entry{
\TA(P,\xabs{s})=[t_1,t_2]\\
% update and check local control
\Gamma_{l,1}=[\coreid\mapsto\Gamma_l(\coreid) - t_2]_{\coreid\in\dom(\Gamma_l)}\\
% update delegated control
\Gamma_d'=\{(\coreid,(\mathit{fid}, t_1'-t_2, t_2'-t_1, t_3)) \sht (\coreid,(\mathit{fid}, t_1', t_2', t_3))\in\Gamma_d \land \neg \cfispositive(t_2'-t_1))\}\\ % \cfispositive(t_1-t_2') TODO: must be strictly positive. Well, maybe we can things that are unsure in d' (i.e., neg \cfispositive(t_2'-t_1)) and while time passes we are always more sure that we are far away from infinite. In that case cfispositive always is positive or null! Everyting works fine. I'm impressed.
\Gamma_{l,2}=\left\{(\coreid, \getanncontrolled(\xabs{C.m})-(t_3-(t_1'-t_2))) \sht
  \begin{array}{c}(\coreid,(\mathit{fid}, t_1', t_2', t_3))\in\Gamma_d \\\land \cfispositive(t_2'-t_1) \land \coreid=\xabs{x.m} \\\land \mathit{type}(x)=\xabs{C} \end{array}\right\}\\
\Gamma_l'=\Gamma_{l,1}\uplus \Gamma_{l,2}\\
\forall \coreid\in\dom(\Gamma_l'),\,\cfispositive(\Gamma_l'(\coreid))
}{\Gamma_l,\Gamma_d\typep_P^{\mathit{t}}\xabs{s}\typed \Gamma_l',\Gamma_d'}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% rhs
\axiom{\Gamma_l,\Gamma_d\typep_P \xabs{e}\typed \emptyset, \Gamma_l,\Gamma_d}
\and
\entry{
  M = \{\xabs{m}\sht \xabs{C.m}\in\dom(\getanncontrolled)\}\\
  S=[\xabs{m}\mapsto \getanncontrolled(\xabs{C.m})]_{\xabs{m}\in M}
}{\Gamma_l,\Gamma_d\typep_P^{\mathit{nt}} \xabs{T x = new C(e$_1$,$\dots$,e$_n$)} \typed S, \Gamma_l,\Gamma_d}
\and
\axiom{\Gamma_l,\Gamma_d\typep_P \xabs{e.get}\typed \emptyset, \Gamma_l,\Gamma_d}
\and
\entry{
  \forall 1\leq i\leq n,\,\mathit{type}(\xabs{e}_i)=\xabs{T}_i\\ % type each expression
  % update \Gamma with the call
  \xabs{e}_1.\xabs{m}\in\dom(\Gamma_l)\Rightarrow\Gamma_l'=\Gamma_l[\xabs{e}_1.\xabs{m}]=\getanncontrolled(\xabs{T$_1$.m})\\
  \xabs{e}_1.\xabs{m}\not\in\dom(\Gamma_l)\Rightarrow\Gamma_l'=\Gamma_l\\
  % update \Gamma with the control delegation
  \getanncontrolling(\xabs{T$_1$.m})=[\xabs{x}_i.\xabs{m}_j\mapsto[t_{i,j}, t_{i,j}']]_{i\in I\subseteq[2..n], j\in J_i}\\
  \exists \Gamma_l'',t_{i,j}'',\,\Gamma_l'=\Gamma_l''\uplus[\xabs{e}_i.\xabs{m}_j\mapsto t_{i,j}'']\ \text{with}\ \cfispositive(t_{i,j}'' - t_{i,j})\\
  c=\{P\sht P\in\tapreds\land P(\xabs{C.m}, \xabs{e}_2,\dots,\xabs{e}_n)\}\\
  t_1=\min(\{ t\sht P\in c,\,\TA(P)=[t,t']\})\\
  t_2=\max(\{ t'\sht P\in c,\,\TA(P)=[t,t']\})\\
  \mathit{fid}\ \text{\rm fresh}
}{\Gamma_l,\Gamma_d\typep_P \xabs{e$_1$!m(e$_2$,$\dots$,e$_n$)} \typed \emptyset, \Gamma_l'',\Gamma_d[\xabs{e}_i.\xabs{m}_j\mapsto (\mathit{fid}, t_1, t_2, t_{i,j}')]}
\end{rules}
\caption{Example of Typing Rules}\label{fig:ts-subset}
\end{figure}

 and $ii)$ use this analysis to check that methods are correctly calledcheck the time validity of every method in a {\tt HABS} program, i.e., check that the time taken by the statements between two methods call
% need to add a join sentence

Interestingly, resource analysis, and time analysis in particular, have already been defined for {\tt ABS}~\cite{DBLP:conf/pepm/AlbertAGGP12,AlbertBHJSTW14,DBLP:journals/jlp/LaneveLPR19} and it is reasonable to imagine that other time analysis, with different capabilities, will be defined in the future.
% reference to our previous paper on time analysis (and maybe others), and motivate the fact that we use a modular approach: many improvements on these analysis is still possible, and checking when methods are called is actually independent to how time is analyzed.
% discuss the modular structure of the type system
% show some rules
% theorem (staetment)






To illustrate our type system, we informally describe some of its typing rules.
The rules are given in Figure~\ref{fig:ts-subset}.

Every node of the AST is tagged, and we have getters on the nodes.
$\tapreds$, $\getanncontrolling$ and $\getanncontrolled$, $\TA{\text{\sf Prgm}}$, $\cfispositive$, $\cfisinfty$, $\mathit{type}$
\begin{figure}
\begin{rules}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% method declaration
\entry{
  \getanncontrolling(\xabs{C.m})=[\xabs{x}_i.\xabs{m}_j\mapsto[t_{i,j}, t_{i,j}']]_{i\in I\subseteq[1..n], j\in J_i}\\ % get controlling annotation from the method
  \getanncontrolled(\xabs{T}_i.\xabs{m}_j)=t_{i,j}''\\ % get controlled annotation from the method
  %\forall 1\leq i\leq n,\, \forall \xabs{m}\ \text{method of}\ \xabs{T}_j,\, % all ceid that need control are controlled
  %  ((\exists j\in J_i,\,\xabs{m}=\xabs{m}_j) \lor (\xabs{T}_i.\xabs{m}\not\in\dom(\getanncontrolled))\\
  \forall \xabs{x}_i.\xabs{m}_j,\, \cfispositive(t_{i,j}'' - t_{i,j}) \\ % check that the initial delay is ok
  % type the method for all its possible execution context
  c=\{P\sht P\in\tapreds\land\exists \xabs{e}_1,\dots,\xabs{e}_n,\,P(\xabs{C.m}, \xabs{e}_1,\dots,\xabs{e}_n)\}\\
  \forall P\in c,\left(\begin{array}{c}
  [\xabs{x}_i.\xabs{m}_j:t_{i,j}]_{i\in I\subseteq[1..n], j\in J_i},\emptyset\typep_P \xabs{s} \typed 
    [\xabs{x}_i.\xabs{m}_j:t_{i,j}^P]_{i_P\in I^P, j_P\in J_i^P},\emptyset\\ I^P\subseteq I \and J_i^P\subseteq J_i\\
  \forall \xabs{x}_i.\xabs{m}_j,\, \cfispositive(t_{i,j}' - (t_{i,j}''-t_{i,j}^P)) % check that the final delay is ok for all possible execution
  \end{array}\right)
}{\xabs{C}\typep\xabs{T m(T$_1$ x$_1$, $\dots$, T$_n$ x$_n$) \{s;return e;\}}}
\and
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% can remove \infty from effect
\entry{
  \Gamma_l,\Gamma_d\typep_P \xabs{s}\typed [\coreid_i\mapsto t_i]\uplus[\coreid\mapsto t],\Gamma_d' \and \cfisinfty(t)
 }{\Gamma_l,\Gamma_d\typep_P \xabs{s}\typed [\coreid_i\mapsto t_i],\Gamma_d'}
 \and
\entry{
  \Gamma_l,\Gamma_d\typep_P \xabs{s}\typed \Gamma_l',[\coreid_i\mapsto (\mathit{fid}_i, t_{i,1}, t_{i,2}, t_{i,3})]\uplus[\coreid\mapsto (\mathit{fid}, t_1, t_2, t_3)] \and \cfisinfty(t_1)
 }{\Gamma_l,\Gamma_d\typep_P \xabs{s}\typed \Gamma_l',[\coreid_i\mapsto (\mathit{fid}_i, t_{i,1}, t_{i,2}, t_{i,3})]}
 \and
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% statements
\entry{
  \Gamma_l,\Gamma_d\typep_P \xabs{s}_1\typed \Gamma_{l,1},\Gamma_d'\\
  \Gamma_l,\Gamma_d\typep_P \xabs{s}_2\typed \Gamma_{l,2},\Gamma_d'\\
  \dom(\Gamma_{l,1})=\dom(\Gamma_{l,2})\\
  \Gamma_l'=[\coreid\mapsto\min(\Gamma_{l,1}(\coreid), \Gamma_{l,2}(\coreid))]_{\coreid\in\dom(\Gamma_{l,1})}
}{\Gamma_l,\Gamma_d\typep_P \xabs{if(e) \{ s$_1$\} else \{ s$_2$ \}}\typed\Gamma_l',\Gamma_d'}
\and
%
\entry{
  \Gamma_l,\Gamma_d\typep_P \xabs{s}_1\typed \Gamma_l',\Gamma_d'\\
  \Gamma_l',\Gamma_d'\typep_P \xabs{s}_2\typed \Gamma_l'',\Gamma_d''
}{\Gamma_l,\Gamma_d\typep_P \xabs{s$_1$ ; s$_2$}\typed\Gamma_l'',\Gamma_d''}
\and
\entry{
  \Gamma_l,\Gamma_d\typep_P^{\mathit{t}} \xabs{await g}\typed \Gamma_l',\Gamma_d'
}{\Gamma_l,\Gamma_d\typep_P \xabs{await g}\typed\Gamma_l',\Gamma_d'}
\and
\entry{
  \Gamma_l,\Gamma_d\typep_P \xabs{rhs}\typed [\xabs{m}_i\mapsto t_i]_{i\in I},\Gamma_l',\Gamma_d'\\
  \Gamma_l''=\Gamma_l'\uplus[\xabs{x.m}_i\mapsto t_i]_{i\in I}\\
  \Gamma_l'',\Gamma_d'\typep_P^{\mathit{t}} \xabs{T x = rhs}\typed \Gamma_l''',\Gamma_d''
}{\Gamma_l,\Gamma_d\typep_P \xabs{T x = rhs}\typed\Gamma_l''',\Gamma_d''}
\and
\entry{
  \Gamma_l,\Gamma_d\typep_P^{\mathit{t}} \xabs{duration(e)}\typed \Gamma_l',\Gamma_d'
}{\Gamma_l,\Gamma_d\typep_P \xabs{duration(e)}\typed\Gamma_l',\Gamma_d'}
\and
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% statement that take time
\entry{
\TA(P,\xabs{s})=[t_1,t_2]\\
% update and check local control
\Gamma_{l,1}=[\coreid\mapsto\Gamma_l(\coreid) - t_2]_{\coreid\in\dom(\Gamma_l)}\\
% update delegated control
\Gamma_d'=\{(\coreid,(\mathit{fid}, t_1'-t_2, t_2'-t_1, t_3)) \sht (\coreid,(\mathit{fid}, t_1', t_2', t_3))\in\Gamma_d \land \neg \cfispositive(t_2'-t_1))\}\\ % \cfispositive(t_1-t_2') TODO: must be strictly positive. Well, maybe we can things that are unsure in d' (i.e., neg \cfispositive(t_2'-t_1)) and while time passes we are always more sure that we are far away from infinite. In that case cfispositive always is positive or null! Everyting works fine. I'm impressed.
\Gamma_{l,2}=\left\{(\coreid, \getanncontrolled(\xabs{C.m})-(t_3-(t_1'-t_2))) \sht
  \begin{array}{c}(\coreid,(\mathit{fid}, t_1', t_2', t_3))\in\Gamma_d \\\land \cfispositive(t_2'-t_1) \land \coreid=\xabs{x.m} \\\land \mathit{type}(x)=\xabs{C} \end{array}\right\}\\
\Gamma_l'=\Gamma_{l,1}\uplus \Gamma_{l,2}\\
\forall \coreid\in\dom(\Gamma_l'),\,\cfispositive(\Gamma_l'(\coreid))
}{\Gamma_l,\Gamma_d\typep_P^{\mathit{t}}\xabs{s}\typed \Gamma_l',\Gamma_d'}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% rhs
\axiom{\Gamma_l,\Gamma_d\typep_P \xabs{e}\typed \emptyset, \Gamma_l,\Gamma_d}
\and
\entry{
  M = \{\xabs{m}\sht \xabs{C.m}\in\dom(\getanncontrolled)\}\\
  S=[\xabs{m}\mapsto \getanncontrolled(\xabs{C.m})]_{\xabs{m}\in M}
}{\Gamma_l,\Gamma_d\typep_P^{\mathit{nt}} \xabs{T x = new C(e$_1$,$\dots$,e$_n$)} \typed S, \Gamma_l,\Gamma_d}
\and
\axiom{\Gamma_l,\Gamma_d\typep_P \xabs{e.get}\typed \emptyset, \Gamma_l,\Gamma_d}
\and
\entry{
  \forall 1\leq i\leq n,\,\mathit{type}(\xabs{e}_i)=\xabs{T}_i\\ % type each expression
  % update \Gamma with the call
  \xabs{e}_1.\xabs{m}\in\dom(\Gamma_l)\Rightarrow\Gamma_l'=\Gamma_l[\xabs{e}_1.\xabs{m}]=\getanncontrolled(\xabs{T$_1$.m})\\
  \xabs{e}_1.\xabs{m}\not\in\dom(\Gamma_l)\Rightarrow\Gamma_l'=\Gamma_l\\
  % update \Gamma with the control delegation
  \getanncontrolling(\xabs{T$_1$.m})=[\xabs{x}_i.\xabs{m}_j\mapsto[t_{i,j}, t_{i,j}']]_{i\in I\subseteq[2..n], j\in J_i}\\
  \exists \Gamma_l'',t_{i,j}'',\,\Gamma_l'=\Gamma_l''\uplus[\xabs{e}_i.\xabs{m}_j\mapsto t_{i,j}'']\ \text{with}\ \cfispositive(t_{i,j}'' - t_{i,j})\\
  c=\{P\sht P\in\tapreds\land P(\xabs{C.m}, \xabs{e}_2,\dots,\xabs{e}_n)\}\\
  t_1=\min(\{ t\sht P\in c,\,\TA(P)=[t,t']\})\\
  t_2=\max(\{ t'\sht P\in c,\,\TA(P)=[t,t']\})\\
  \mathit{fid}\ \text{\rm fresh}
}{\Gamma_l,\Gamma_d\typep_P \xabs{e$_1$!m(e$_2$,$\dots$,e$_n$)} \typed \emptyset, \Gamma_l'',\Gamma_d[\xabs{e}_i.\xabs{m}_j\mapsto (\mathit{fid}, t_1, t_2, t_{i,j}')]}
\end{rules}
\caption{Example of Typing Rules}\label{fig:ts-subset}
\end{figure}

 and $ii)$ use this analysis to check that methods are correctly calledcheck the time validity of every method in a {\tt HABS} program, i.e., check that the time taken by the statements between two methods call
% need to add a join sentence

Interestingly, resource analysis, and time analysis in particular, have already been defined for {\tt ABS}~\cite{DBLP:conf/pepm/AlbertAGGP12,AlbertBHJSTW14,DBLP:journals/jlp/LaneveLPR19} and it is reasonable to imagine that other time analysis, with different capabilities, will be defined in the future.
% reference to our previous paper on time analysis (and maybe others), and motivate the fact that we use a modular approach: many improvements on these analysis is still possible, and checking when methods are called is actually independent to how time is analyzed.
% discuss the modular structure of the type system
% show some rules
% theorem (staetment)


\paragraph{Formalization}

For simplicity, we suppose that all statements in a program syntax are distinct (e.g., by adding a hidden counter on them), so that the time analysis can give the time of every statement and not get confused if two identical statements are called in a different context (with different effects).

\begin{definition}
A {\em Counting Framework} is a tuple $\CF=(\cfexps,\cfminus,\cfisinfty,\cfispositive)$ where:
 $\cfexps$ is the set of all counting expressions;
 $\cfminus:(\cfexps\times\cfexps)\rightarrow\cfexps$ is the minus operation;
 $\cfisinfty\subseteq\cfexps$ is a predicate over counting expressions stating which ones are known to correspond to infinity;
 and $\cfispositive\subseteq\cfexps$ is a predicate over counting expressions stating which ones are known to be positive or null.
% TODO: find a sentence to say that the CF and its elements are set and global
A {\em Time Analysis} (TA) for a program {\sf Prgm} is a tuple $\TA{\textsf{Prgm}}=(\CF,\tapreds,\tamap)$ where:
 $\CF=(\cfexps,\cfminus,\cfisinfty,\cfispositive)$ is a counting framework;
 % $e_{\min}$ (resp. $e_{\max}$) is an expression of $\CF$, giving the minimum (resp. maximum) time the init block takes to execute;
 $\tapreds\subseteq(\prgnames\times e^\infty)$ is a set of predicates over lists of values tagged with a method name or {\tt init};
 and $\tamap:(\tapreds\cup\tapreds\times\prgstatmts)\mapsto(\cfexps\times\cfexps)$ is a partial function from
  predicates in $\tapreds$ or pairs of predicates and statements in {\sf Prgm}, to pairs of counting expressions.
\end{definition}


\begin{notation}
Given a trace $\theta$ and a time $t$, we write $\mathit{cn}\in\theta(t)$ iff there exists $\mathit{tcn}$ such that $\theta(t)=\mathit{tcn}\ \mathit{cn}$.
Moreover, we write $\mathit{cn}\in\theta$ iff there exists $t$ such that $\mathit{cn}\in\theta(t)$.

We write $(\tau,\mathit{fid},\xabs{rs})\in\theta(t)$ iff there exists $o$, $\xabs{C}$, $\rho$, ${\mathit{ODE}, f}$ and $q$
 such that $(o, \xabs{C}, \rho, {\mathit{ODE}, f}, (\tau,\mathit{fid},\xabs{rs}), q)\in\theta(t)$.
Finally, we write $(\tau,\mathit{fid},\xabs{rs})\in\theta$ iff there exists $t$ such that $(\tau,\mathit{fid},\xabs{rs})\in\theta(t)$.
\end{notation}

\begin{definition}
Given a type analysis $\TA{\textsf{Prgm}}=(\CF,\tapreds,\tamap)$,
 a {\em timed instance} $\TI$ is a partial function from future names to predicates in $\tapreds$ such that $\xabs{init}\in\TI(\mathit{fid}_{\mathit{init}})$.

A time analysis $\TA{\textsf{Prgm}}=(\CF,\tapreds,\tamap)$ is {\em method-valid} for a trace $\theta$ iff
 for all $t_1$ and all $\mathsf{msg}(o, \xabs{m}, \many{\xabs{e}}, \mathit{fid})\ (o, \xabs{C}, \rho, {\mathit{ODE}, f}, \mathit{prc}, q)\in\theta(t_1)$:
\begin{enumerate}
\item the set $\{P\sht P\in\tapreds\land P(\xabs{C.m}, \many{\xabs{e}})\}$ is a singleton; let write $P$ its element;
\item and writing $\tamap(P)=(e_{\min}, e_{\max})$ there exists $t_2$ with $\mathsf{fut}(fid, \xabs{e})\in\theta(t_2)$,
  $\cfispositive(e_{\max} - (t_2-t_1))$ and $\cfispositive((t_2-t_1) - e_{\min})$
\end{enumerate}

A time analysis $\TA{\textsf{Prgm}}=(\CF,\tapreds,\tamap)$ is {\em statement-valid} for a trace $\theta$ iff there exist a timed instance $\TI$ such that,
 given any process $(\tau,\mathit{fid},\xabs{rs})\in\theta$ with $\xabs{rs}=\xabs{r;rs'}$, we have $\mathit{fid}\in\dom(\TI)$ and,
  writing $\tamap(\TI(\mathit{fid}),\xabs{r})=(e_{\min}, e_{\max})$:
\begin{enumerate}
\item for all $t_1$ and $t_2$ with $(\tau,\mathit{fid},\xabs{s;rs})\in\theta(t_1)$ and $(\tau,\mathit{fid},\xabs{rs})\in\theta(t_2)$,
  we have that $\cfispositive(e_{\max} - (t_2 - t_1))$
\item there exists $t_1$ and $t_2$ with $(\tau,\mathit{fid},\xabs{rs})\in\theta(t_1)$ and $(\tau,\mathit{fid},\xabs{rs})\in\theta(t_2)$
  such that $\cfispositive(e_{\min} - (t_2 - t_1))$
\item there exists $\mathsf{msg}(o, \xabs{m}, \many{\xabs{e}}, \mathit{fid})\ (o, \xabs{C}, \rho, {\mathit{ODE}, f}, \mathit{prc}, q)\in\theta$
  with $(\mathsf{C.m}, \many{\xabs{e}})\in\TI(\mathit{fid})$ and $\texttt{\#}(\{P\sht P\in\tapreds\land(\xabs{C.m}, \many{\xabs{e}})\in P\})=1$
\end{enumerate}

A time analysis $\TA{\textsf{Prgm}}$ is {\em valid} iff it is method- and statement-valid for all the possible traces of its program {\sf Prgm}.
\end{definition}



\mltodoin{content goes here}










\begin{rules}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% statement that take time
\entry{
\TA(c,\xabs{s})=[t_{\min},t_{\max}]\\
% update
\Gamma_{l,1}=[\coreid\mapsto\Gamma_l(\coreid) - t_{\max}]_{\coreid\in\dom(\Gamma_l)}\\
% split delegated
C=\{\coreid\mid\coreid\in I\land t_\coreid^2<t_{\min}\}\\
%
\Gamma_d'=[\coreid\mapsto(\mathit{fid}, t_\coreid^1-t_{\max}, t_\coreid^2-t_{\min}, t_\coreid^3)]_{\coreid\in \dom(\Gamma_d)\setminus C}\\
\Gamma_{l,2}=[\coreid\mapsto t_\coreid^3 + (t_{\max}-t_\coreid^1)]_{\coreid\in C}\\
% combine and check
\Gamma_l'=\Gamma_{l,1}\uplus \Gamma_{l,2}\and
\forall \coreid\in\dom(\Gamma_l'),\,\Gamma_l'(\coreid) \geq 0
}{\Gamma_l,[\coreid\mapsto(\mathit{fid}, t_\coreid^1, t_\coreid^2, t_\coreid^3]_{\coreid\in I}\typep_c^{\mathit{t}}\xabs{s}\typed \Gamma_l',\Gamma_d'}
\end{rules}

==> externacq.tex <==
The last section introduced external control for timed post-regions, where interaction between controlled method and controlling environment is synchronized through global time.
Next, we investigate external control for event-based post-regions. 
This requires more elaborate structures: as the state of a HAO is strongly encapsulate, an external process cannot synchronize on a boolean condition.
Thus, there is no language-mechanism to react without delay to an event from another Active Object and any such language feature would destroy the compositionality properties of Active Objects.

Our solution is a generalization of a pattern first employed in the \texttt{FormbaR} model of railway operations~\cite{scp}, illustrated in the code below:

\noindent\begin{abscode}
class Signal(Int i){
    Unit acq(){ await i == 10; }
    Unit reset(){ i = 0; }
    Unit setI(Int j){ i = j;} 
}

class Monitor(Signal s){
    {
        while(true){
            Fut<Unit> f = s!acq();
            await f?;
            Fut<Unit> f2 = s!reset();
            f2.get;
        }
    }
}
\end{abscode}

The \abs{acq} method reacts to an event \emph{inside} the controlled class. The \abs{Monitor} instance synchronizes on this method -- as synchronization is instant, it can reschedule its process \emph{immediatelly} and reset the \abs{Signal} instance. The value of \abs{i} is always below 10 (if initialized below 10).
This requires, however several additional properties:
\begin{itemize}
\item To react immediatelly, the monitor may not block during a time advance. 
\item To ensure that the value of \abs{i} is indeed always below 10, no other object than the controlling \abs{Monitor} instance may call \abs{setI}.
\item The monitor may not store the future for \abs{acq} or call several processes of this method.
\end{itemize}
If these properties hold, and there is always some process synchronizing on a running \abs{acq} process, 
then we may regard \abs{acq} as the trigger of an \emph{event} controller and add its guard to the post-region boundary. 
The controlling code itself is in \abs{setI} which may assume that the trigger of \abs{acq} holds.

As with timed post-regions, we give a rely on ideas from type systems and check the required properties statically with a different type system.
This type system has similarities with \emph{ownership} type....


We again give an adjusted room controller.
\begin{example}







\ektodoin{NONOVERLAPPING + SCHEDULING POLICY}




\begin{figure}
\begin{abscode}
class Tank(){
    physical Real temp = 20;
    Real power = -0.5;
    physical{ temp' = power; }
    /*@ lingering checkUp @*/
    Unit acqUp(){ await diff temp >= 23.5 && power > 0; }

    Fut<Unit> checkUp(){
        power = -0.5;
        return this!acqUp();
    }

    /*@ lingering checkDown @*/
    Unit acqDown(){ await diff temp <= 17.5 && power < 0; }
   
    Fut<Unit> checkDown(){
        power = 0.5;
        return this!acqDown();
    }
}
\end{abscode}
\caption{caption}
\label{fig:caption}
\end{figure}
\end{example}

\paragraph{Type System}
\mltodoin{content goes here}
\paragraph{Proof System}
For event-based external control, we need to slightly modify our proof scheme: we assume the guard of the acquisition method as the guard of the lingering method.
\begin{theorem}
Let \texttt{C} be a class with a an acquisition-lingering pair \abs{acq-m}, \abs{lin-m}. 
Let \abs{g} be the guard of \abs{acq-m}
The externally controlled event post-region of is defined as follows:
\[\psi^\xabs{acq-m}_\xabs{lin-m} \equiv \widetilde{\neg}\xabs{g}\]
Let $\mathbf{Prgm}^\vdash$ be the set of well-typed programs according to Def.~\ref{def:type1}.
\begin{itemize}
    \item 
The post-region $\psi^\xabs{acq-m}_\xabs{lin-m}$ is sound for $\mathbf{Prgm}^\vdash$.
    \item 

The proof obligation scheme remains sound if \abs{g} is added to the pre-condition of \abs{lin-m} and no proof obligation is generated for \abs{acq-m}.
\end{itemize}
\end{theorem}
\ektodoin{explain + example}

==> habs_old.tex <==
In this section we present the preliminiaries for the rest of the article.
First, we present the \emph{Hybrid Abstract Behavioral Specification} (\texttt{HABS}) language that implements Hybrid Active Objects.
We only present the language parts that are relevant for post-region based verification and omit, e.g., inheritance, method visibility and variability.
A complete description is given in~\cite{arxiv}.
We refrain from introducing full \texttt{HABS} and omit, e.g., inheritance. 


A hybrid active object (HAO) is a strongly encapsulated object, i.e., 
no other object, not even from the same class, may access the fields of an instance. Communication between HAOs is only possible through asynchronous method calls and synchronization: each method call generates a container called \emph{future} for the caller that uniquely identifies the (to-be) started process at callee side. The future may be passed around and permits to synchronize (i.e., wait until the called process terminates) with it and read the return value of the associated process.
HAOs implement \emph{cooperative scheduling}:
Inside an object, only one process is active at a time. This process cannot be preempted by the scheduler --- 
it must explicitly release control by either terminating or suspending (via \abs{await}). 
These two properties make (hybrid) active objects easy to analyze: 
approaches for sequential program analyses can be applied
between two \abs{await} statements (and method start and end).

\begin{figure}[bt]
\noindent\begin{abscode}
class Tank(Log log){                //class header with field declaration
  physical Real level = 5;          //field declaration
  Real drain = -1;                 //field declaration
  physical{ level' = drain; }       //dynamics
  { this!up(); this!down(); }$\label{line:init}$        //constructor
  Unit down(){                     //method header
    await diff level <= 3 & drain <= 0;
    log!triggered(); drain =  1; this!down();
  }
  Unit up(){                       //method header
    await diff level >= 10 & drain >= 0;
    log!triggered(); drain = -1; this!up();
  }
}
\end{abscode}
\caption{A water tank in \HABS with event-based control.}
\label{fig:bball}
\end{figure}

Hybrid Active Objects differ from standard Active Objects by a \abs{phyiscal} block and \abs{physical} fields\footnote{The variant of \texttt{HABS} presented here differs slightly in the syntax of the \abs{physical} block from~\cite{arxiv}. The difference is only whether \abs{physical} fields are declared within the \abs{physical} block with the ODEs or outside of it.}.
A \abs{physical} field is a field that has some dynamics, the  \abs{physical} block describes the dynamics of all  \abs{physical} fields as ODEs.
This dynamics are used to change the state whenever time advances. 
Inside a method, an imperative language is used, which has special statements to advance time or wait until some condition on the state holds.
These conditions define an urgent transition: the method is reactivated as soon as possible once the condition holds. Urgent semantics simplify simulation and \texttt{HABS} is specifically designed to combine modeling, simulation, analysis and verification.



Before we give the formal syntax and semantics, we illustrate \texttt{HABS} with the following example.
\begin{example}\label{ex:eventroom}
Consider the water tank model in Fig.~\ref{fig:bball}.
The tank keeps a water level between 3 and 10.
The pictured class, \abs{Tank} has two discrete fields (\abs{log} and \abs{drain}) and
a \abs{physical} field \abs{level}.
A physical field is described by its initial value and am ODE in the \abs{physical} block, which models that the water level is linear with respect to the drain.
Line~\ref{line:init} gives the constructor in form of an initialization block where the two methods 
\abs{up} and \abs{down} are called.
Each method starts with a statement that has as its guard the condition when the process will be scheduled (for \abs{up}, at the moment the level reaches 10 while water rises). 
This is logged by calling the external object  \abs{log} on method \abs{triggered}.
This method call is asynchronous, i.e., the execution of the \abs{up} (or \abs{down}) continues without waiting for it to finish. No future is generated in this example. 
Then, the drain is adjusted and the methods calls itself recursively to react the next time.
\end{example}

The above example illustrates \emph{event-based} control, as the guards of the \abs{await diff} statement define an event boundary. Alternatively, one may use \emph{time-based} control, as the following example illustrates.

\begin{example}\label{ex:timedroom}
The controller in Fig.~\ref{fig:ctank} checks the water level of a tank every $\frac{1}{2}$ seconds by using the \abs{await duration} statement to suspend the \abs{ctrl} process for the required amount of time.
\begin{figure}[b!th]
\begin{abscode}
class TankTick(Real inVal){
  physical Real level = 5;
  Real drain = -0.5;
  physical{ level' = drain; }
  { this!ctrl(); }
  Unit ctrl(){
    await duration(1/2);
    if(level <= 3.5) drain =  0.5;
    if(level >= 9.5) drain = -0.5;
    this!ctrl();
  }
}
\end{abscode}
\caption{A water tank in \HABS with time-based control.}
\label{fig:ctank}
\end{figure}
\end{example}














\subsection{Syntax}


The syntax of \HABS is given by the grammar in Fig.~\ref{fig:syntax}.
Standard expressions \texttt{e} are defined over fields \texttt{f}, variables \texttt{v} and
operators \texttt{!}, \texttt{|}, \texttt{\&}, \texttt{>=}, \texttt{<=}, \texttt{+}, \texttt{-},
\texttt{*}, \texttt{/}.  
Ordinary differential expressions (ODEs) \abs{ODE} are equalities over expressions extended with a derivation operator \abs{e'}.
Types \texttt{T} are all class names, type-generic
futures \abs{Fut<T>}, \abs{Real}, \abs{Unit} and \abs{Bool}. 

\begin{figure*}[tbh]
\resizebox{\textwidth}{!}{
\begin{minipage}{1\textwidth}
\begin{align*}
\mathsf{Prgm} ::=~& \many{\mathsf{CD}}~\{\mathsf{s}\}\quad
\mathsf{CD} ::= \xabs{class C}\left[\xabs{(}\many{\xabs{T f}}\xabs{)}\right]\{\many{\mathsf{FD}}~[\mathsf{Phys}]~[\{\mathsf{s}\}]~\many{\mathsf{Mt}}\} 
&& \text{\small Classes}\\
\mathsf{Mt} ::=~& \xabs{T m(}\many{\xabs{T}~\xabs{v}}\xabs{)}~\{\mathsf{s}\xabs{;}\xabs{return e;}\}
&& \text{\small Methods}\\
\mathsf{FD} ::=~& \xabs{T f[ = e];} \synsep  \xabs{physical Real f = e;}
&& \text{\small Fields}\\
\mathsf{Phys} ::=~& \xabs{physical}~\{\many{\mathsf{ODE}}\} 
&&\text{\small Physical Block}\\
%\midrule
%\midrule
\mathsf{s} ::=~&
\xabs{while (e)}~\{\mathsf{s}\}\synsep
\xabs{if (e)}~\{\mathsf{s}\}~[\xabs{else}~\{\mathsf{s}\}]\synsep
\mathsf{s}\xabs{;}\mathsf{s} && \\
&\synsep\xabs{await}~\mathsf{g} \synsep
[[\xabs{T}]~\xabs{e}] = \mathsf{rhs} \synsep \xabs{duration(e)}&&\text{\small Statements}\\
\mathsf{g} ::=~&\xabs{e?} \synsep \xabs{duration(e)} \synsep \xabs{diff e}
&&\text{\small Guards}\\
\mathsf{rhs} ::=~&
\xabs{e} \synsep \xabs{new C(}\many{\xabs{e}}\xabs{)} \synsep 
\xabs{e.get} \synsep
\xabs{e!m(}\many{\xabs{e}}\xabs{)}
&&\text{\small RHS Expressions}
\end{align*}
\end{minipage}
}
\caption{\HABS grammar. Notation $[\cdot]$ denotes optional elements and $\many{~\cdot~}$ lists.}
\label{fig:syntax}
\end{figure*}

A program consists of a main block and a set of classes. Each class may have a list of discrete fields that are passed as parameters on object creation and a list of internally declared fields with.
An internally declared field\footnote{\emph{All} fields, independent of where they are declared, are accessible only from their object.} may be declared as \abs{physical}. In this case it must be of \abs{Real} type and  must be initialized.
Furthermore, a class has an optional physical block, which defines the dynamics of \abs{physical} fields and an optional
initialization block that is executed directly after object creation and serves as the constructor. Lastly, a class has a set of methods. All methods are accessible from the outside.

Methods, initializing and main block consist of statements. Besides the asynchronous method calls (\texttt{e!m()}) described above, only the following are non-standard:
\begin{itemize}
\item The \abs{duration(e)} statement advances time by \texttt{e} time units. No other process may execute during this advance.
\item The \abs{e.get} statement reads from a future. A future is a container that is generated by an asynchronous call. 
Afterwards a future may be passed around. With the \abs{statement} one can read the return values once the called process terminates. Until then, the reading process blocks and no other process can run on the object.
\item The \abs{await g} statement suspends the process until the guard \texttt{g} holds. 
A guard is either (1) a future poll \texttt{e?} that determines whether the call for the future in \texttt{e} has terminated, (2) a duration guard that advances time while \emph{unblocking} the object or (3) a differential guard that holds once expression \texttt{e} holds.
\end{itemize}


We assume that all methods are suspension-leading, i.e., each method starts with an \abs{await} statement. This is easily achieved by adding \abs{await diff true} if a method is not suspension-leading without changing the behavior.
Concerning the \abs{physical} block, we only admit blocks describing trivial behavior for all \abs{physical} field.
Finally, we only consider well-typed (w.r.t.\ data types) programs where differential guards contain only \abs{Real}-typed variable. Note that expressions are not defined over strong inequalities. 



\subsection{Semantics}

The Semantics of a program run is defined as a trace, extracted from a transition sequence defined in Plotkin-style structural operational semantics~\cite{plotkin} (SOS).
At each point in time, the SOS semantic defines the state and the current global time of the program as a \emph{configuration}.
The transition system is defined by a set of conditional rewrite rules over the configurations.
Finally, the trace of a run is extracted by filling-in the gaps between the points in time where the rewrite rules generate a configuration.

To represent the state of a program, we extend the syntax of statements to \emph{runtime syntax}, which also incorporates a \abs{suspend} statement, which deschedules a process.  
The \HABS semantics are SOS semantics and are using standard SOS notation, except that (1) we use the timed extension of Bj{\o}rk et al.~\cite{BjorkBJST13}, which allows
us to keep track of time in the semantics, and (2) that time advance changes not only the time, but also the object state, because it evolves according to the \abs{physical} block.
We only present the rules relevant for the hybrid extension of \texttt{ABS} here, for the missing rules we refer to the semantics of timed \texttt{ABS} by Bj{\o}rk et al.~\cite{BjorkBJST13}, whose semantics we conservatively extend~\cite{arxiv}: if no \abs{physical} block is used, then our semantics is the same as the one for timed \texttt{ABS}.

\begin{figure}[tbh]
\begin{align*}
\mathit{tcn} &::= \mathsf{clock}(\xabs{e})~\mathit{cn}\qquad
\mathit{cn} ::= \mathit{cn}~\mathit{cn} \synsep \mathit{fut} \synsep \mathit{msg} \synsep \mathit{ob} \qquad \mathit{fut} ::= \mathsf{fut}(\mathit{fid},\xabs{e})\\
\mathit{msg} &::= \mathsf{msg}(o, \many{\xabs{e}}, \mathit{fid})\qquad
\mathit{ob} ::= (o, \rho, {\mathit{ODE}, f}, \mathit{prc}, q)\qquad q ::= \many{\mathit{prc}}\qquad
\\
\mathit{prc} &::= (\tau,\mathit{fid},\xabs{rs})\synsep\bot\qquad
\xabs{rs} ::= \xabs{s} \synsep \xabs{suspend;s}
\end{align*}
\caption{Runtime syntax of \HABS.}
\label{fig:cfg}
\end{figure}

\begin{definition}[Runtime Syntax~\cite{BjorkBJST13}]\label{def:rsyntax}
The runtime syntax of \HABS is given by the grammar in Fig.~\ref{fig:cfg}. 
Let $\mathit{fid}$
range over future names, $o$ over object identities,
and $\rho,\tau,\sigma$ over stores (i.e., maps from fields or variables
to values). 
\end{definition}



A timed configuration $\mathit{tcn}$ has a clock $\mathsf{clock}$ with
the current time as its parameter \abs{e} of \abs{Real} type and an object
configuration $\mathit{cn}$.  An object configuration 
consists of messages $\mathit{msg}$, futures $\mathit{fut}$ and
objects $\mathit{ob}$.  A message
$\mathsf{msg}(o, \many{\xabs{e}}, \mathit{fid})$ has the callee $o$, passed
parameters $\many{\xabs{e}}$ and the generated future $\mathit{fid}$ as its parameters.  A future
$\mathsf{fut}(\mathit{fid},\xabs{e})$ has as parameters the future name $\mathit{fid}$
with its return value \abs{e}.  An object
$(o, \rho, \mathit{ODE}, f, \mathit{prc}, q)$ has
an identifier $o$, an object store $\rho$, the current dynamic
$f$, an active process $\mathit{prc}$ and a set of inactive
processes $q$ as its parameters.  $\mathit{ODE}$ is taken from the class declaration.  A
process is either terminated ($\bot$) or has the form
$(\tau,\mathit{fid},\xabs{rs})$: the process store $\tau$ with the current state of
the local variables, its future identifier $\mathit{fid}$, and the statement $\xabs{rs}$
left to execute. Composition $\mathit{cn}_1~\mathit{cn}_2$
is commutative and associative. 

We denote the combined local and global store with $\sigma = \rho + \tau$, which is the method composition defined by $\mathbf{dom}(\sigma) = \mathbf{dom}(\rho) \cup \mathbf{dom}(\tau)$, $\forall x \in \mathbf{dom}(\rho).~\sigma(x) = \rho(x)$
and $\forall x \in \mathbf{dom}(\tau).~\sigma(x) = \tau(x)$.


\paragraph{Evaluation of Guards and Expressions.}
To define the transition system underlying the SOS, one must be able to evaluate expressions and guards. 
Additionally to the current store, expressions and guards are evaluated with respect to a given time and continuous dynamics.
This is necessary to compute how much time may advance before a differential guard is evaluated to true. We first introduce the evaluation of expressions.

Given fixed initial values of fields $\rho$ and a local store $\tau$, the solution $f$ of an ODE is unique and $f(0) = \sigma = \rho + \tau$.\ektodo{check uniqueness condition}
Non-physical fields do not evolve.
\begin{definition}[Evaluation of Expressions]
Let $f$ be a mapping from $\mathbb{R}^+$ to stores and $\sigma = f(0)$ the current combined state.
Let $\xabs{f}_p$ be a physical field and $\xabs{f}_d$ a non-physical field.
The semantics of fields $\xabs{f}_p$, $\xabs{f}_d$, unary operators ${\sim}$ and
binary operators
$\oplus$
after $t$ time units is defined as follows:
\begin{align*}
\sem{\xabs{f}_d}_\sigma^{f,t} &= \sigma(\xabs{f}_d) \qquad
\sem{\xabs{f}_p}_\sigma^{f,t} = f(t)(\xabs{f}_p)\\
\sem{{\sim}\xabs{e}}_\sigma^{f,t} &= {\sim}\sem{\xabs{e}}_\sigma^{f,t}\qquad\sem{\xabs{e} \oplus \xabs{e'}}_\sigma^{f,t} = \sem{\xabs{e}}_\sigma^{f,t} \oplus \sem{\xabs{e'}}_\sigma^{f,t}
\end{align*}
\end{definition}

Evaluation of guards is defined in two steps: 
First, the \emph{maximal time elapse} is computed. I.e., the maximal time that may pass without the guard expression evaluating to true
For differential guards \abs{diff e} this is the minimal time until \abs{e} becomes true.
Then, the guard evaluates to true if no time advance is needed.

\begin{definition}[Evaluation of Guards]\label{def:semant-diff-guards}
Let $f$ be a continuous dynamic of object $o$ in state $\sigma$. 
The evaluation of guards \abs{g} is defined as 
\[
\sem{\xabs{g}}_\sigma^{f,0} = \text{\normalfont\text{true}} \iff \mathit{mte}_\sigma^f(\xabs{g}) \leq 0
\]
The maximal time elapse {\normalfont($\mathit{mte}$)} is given in Fig.~\ref{fig:guard}.
\begin{figure}
\scalebox{0.85}{\begin{minipage}{\textwidth}
\begin{align*}
\mathit{mte}_\sigma^f(\xabs{duration(e)}) &= \sem{\xabs{e}}^{f,0}_{\sigma} \quad
\mathit{mte}_{\sigma}^f(\xabs{e?}) = \cased{0 &\text{ if $\sem{\xabs{e}}^{f,0}_\sigma$ is resolved} \\ \infty & \text{ otherwise}}\\
\mathit{mte}_\sigma^f(\xabs{diff e}) &= \argmin_{t\geq 0}\big(\sem{\xabs{e}}_\sigma^{f,t} = \text{\normalfont\text{true}}\big)
\end{align*}
\end{minipage}}
\caption{Computing the Maximal Time Elapse.}
\label{fig:guard}
\end{figure}
\end{definition}

The transition system has two parts: first, the \emph{discrete transition system}, i.e., the rules that operate on object configurations. Then, the \emph{continuous transition system} to handle time and operate on timed configurations.

\begin{figure*}[b!th]
\noindent\scalebox{0.85}{\begin{minipage}{\textwidth}
\begin{align*}
\rulename{1}\ &\big(o, \rho,{\mathit{ODE}, f}, (\tau,\mathit{fid},\xabs{await g;s}), q\big) ~\rightarrow~ \big(o, \rho,{\mathit{ODE}, f}, (\tau,\mathit{fid},\xabs{suspend;await g;s}),q\big)\\
\rulename{2}\ &\big(o, \rho,{\mathit{ODE}, f}, (\tau,\mathit{fid},\xabs{suspend;s}), q\big) ~\rightarrow~ \big(o, \rho,{\mathit{ODE}, \mathsf{sol}(\mathit{ODE},\rho)}, \bot, q\circ(\tau,\mathit{fid},\xabs{s})\big)\\
\rulename{3}\ &\big(o, \rho,{\mathit{ODE}, f}, \bot, q\circ(\tau,\mathit{fid},\xabs{await g;s})) \rightarrow~ \big(o, \rho,{\mathit{ODE}, f}, (\tau,\mathit{fid},\xabs{s}),q\big) \qquad\text{if $\sem{g}_{\rho\circ\tau}^{f,0}$ = \text{\normalfont\text{true}}}\\
\rulename{4}\ &\big(o, \rho,{\mathit{ODE}, f}, (\tau,\mathit{fid},\xabs{v = e;s}), q\big) \\&\rightarrow~ \big(o, \rho,{\mathit{ODE}, f}, (\tau[\xabs{v} \mapsto \sem{\xabs{e}}^{f,0}_{\rho\circ\tau}],\mathit{fid},\xabs{s}),q\big)\qquad
\text{if \xabs{e} contains no call or \abs{get}}\\
\rulename{5}\ &\big(o, \rho,{\mathit{ODE}, f}, (\tau,\mathit{fid},\xabs{return e;}), q\big) \rightarrow~\big(o, \rho,{\mathit{ODE}, \mathsf{sol}(\mathit{ODE},\rho)}, \bot, q\big)~\mathsf{fut}\big(\mathit{fid},\sem{\xabs{e}}^{f,0}_{\rho\circ\tau}\big)\\
\rulename{6}\ &\big(o, \rho,{\mathit{ODE}, f}, (\tau,\mathit{fid},\xabs{v = e.get;s}), q\big)~\mathsf{fut}\big(\mathit{fid},\xabs{e'}\big) 
\\&\rightarrow~ \big(o, \rho,{\mathit{ODE}, f}, (\tau,\mathit{fid},\xabs{v = e';s}), q\big) \qquad\text{if }\sem{\xabs{e}}^{f,0}_{\rho\circ\tau} = \mathit{fid}\\
\rulename{7}\ &\big(o, \rho,{\mathit{ODE}, f}, (\tau,\mathit{fid},\xabs{v = e!m(e}_1,\dots\xabs{e}_n\xabs{;s}), q\big) 
\\&\rightarrow~
\big(o,\rho,{\mathit{ODE},f},(\tau[\xabs{v}\mapsto f'],\mathit{fid},\xabs{s}),q\big) ~\mathsf{msg}\big(\sem{\xabs{e}}^{f,0}_{\rho\circ\tau},(\sem{\xabs{e}_1}^{f,0}_{\rho\circ\tau},\dots,\sem{\xabs{e}_n}^{f,0}_{\rho\circ\tau}),\mathit{fid}_2\big)\qquad\mathit{fid}_2\text{ fresh}
\end{align*}
\end{minipage}}
\caption{Selected rules for the \HABS discrete transition system.}
\label{fig:ntsem}
\end{figure*}

\paragraph{Discrete Transition System}

Fig.~\ref{fig:ntsem} gives the most important rules for the semantics of objects, the omitted rules are given in~\cite{BjorkBJST13}.
The rules match on object configurations and the matching part is rewritten accordingly.
For example, rule \rulename{5} matches on a single object and rewrites it into an object and a future. 

The rule \rulename{1} introduces a \abs{suspend} statement in front of an
\abs{await} statement.  Rule \rulename{2} consumes a \abs{suspend}
statement and moves a process into the queue of its object---at this
point, the ODEs are translated into some dynamics with $\mathsf{sol}$.   
Rule \rulename{3} activates a process
with a following \abs{await} statement, if its guard evaluates to
true. An analogous rule (not shown in Fig.~\ref{fig:ntsem}) activates
a process with any other non-\abs{await} statement.  Rule \rulename{4}
evaluates an assignment to a local variable. The rule for field is
analogous.  
Rule \rulename{5} realizes a termination (with solutions
of the ODEs) and \rulename{6} a future read. Finally, \rulename{7} is
a method call that generates a message.
%, the rule for transforming a message into a process is
%straightforward.

%%%%%%%%%%%%%%%%%%HERE

\paragraph{Continuous Transition System}

For configurations, there are two rules, shown in Fig.~\ref{fig:tsem}.
Rule \rulename{i} realizes a step of an object without advancing
time. Only if \rulename{i} is not applicable, rule \rulename{ii} can
be applied. It computes the global maximal time elapse 
and advances the time in the clock and all objects.  

State change during a time advance is handled functions
$\mathit{adv}$ which are applied to all elements of a configuration
We only give two members of the family: $\mathit{adv}_{\mathit{heap}}$ takes as parameter a store $\sigma$, the dynamics $f$ and a duration $t$, 
$\mathit{adv}_{\mathit{prc}}$ takes a process $\mathit{prc}$, the dynamics $f$ and a duration $t$.
Both advance its first parameter by $t$ time units according to $f$.  
The state evolves according to the current dynamics and the guards of \abs{duration} guards and statements are decreased by $t$ (if the \abs{duration} clause is part of the first statement of an unscheduled process).
For non-hybrid Active Objects $\mathit{adv}_{\mathit{heap}}(\rho,t) = \rho$. For all other cases of \textit{adv}, the function only propagates according to the syntax in definition~\ref{def:rsyntax}.

\begin{figure}[tbh]
\scalebox{0.85}{\begin{minipage}{\columnwidth}
\begin{align*}
\rulename{i}~&\mathsf{clock}(t)~\mathit{cn}~\mathit{cn}' \rightarrow \mathsf{clock}(t)~\mathit{cn}''~\mathit{cn}' \qquad\text{ with } \mathit{cn} \rightarrow \mathit{cn}''\\
\rulename{ii}~&\mathsf{clock}(t)~\mathit{cn} \rightarrow \mathsf{clock}(t+t')~\mathit{adv}(\mathit{cn},t') \qquad\text{ if \rulename{i} is not applicable}\text{ and }\mathit{mte}(\mathit{cn}) = t'\neq \infty
\end{align*}
\end{minipage}}

\scalebox{0.85}{\begin{minipage}{\columnwidth}
\begin{align*}
\mathit{adv}_\mathit{prc}\big((\tau,\mathit{fid},\xabs{s}),f,t\big) &= (\tau,\mathit{fid},\xabs{s}) \text{ if }\xabs{s} \neq (\xabs{await duration(e); s'})\\
\mathit{adv}_\mathit{prc}\big((\tau,\mathit{fid},&\,\xabs{await duration(e);s}),f,t\big) = 
(\tau,\mathit{fid},\xabs{await duration(e+}t\xabs{);s})\\
\mathit{adv}_\mathit{heap}(\rho,f,t)(\xabs{f}) &=
\cased{
\rho(\xabs{f}) & \text{ if \abs{f} is not physical} \\
f(t)(\xabs{f})  & \text{ otherwise }}
\end{align*}
\end{minipage}}
\caption{Timed semantics of \HABS configurations.}
\label{fig:tsem}
\end{figure}

Similarly to \textit{adv}, we need to extend the \textit{mte} function to configurations as follows:

\noindent\scalebox{0.85}{\begin{minipage}{\columnwidth}
\begin{align*}
\mathit{mte}(\mathit{cn}~\mathit{cn}') &= \mathbf{min}(\mathit{mte}(\mathit{cn}),\mathit{mte}(\mathit{cn}'))\qquad\mathit{mte}(\mathit{msg}) = \mathit{mte}(\mathit{fut}) = \infty\\
\mathit{mte}(o, \rho, \mathit{ODE}, f, \mathit{prc}, q) &=\sem{\mathbf{min}_{q' \in q}(\mathit{mte}(q'),\infty)}_\rho\qquad
\mathit{mte}(\tau,\mathit{fid},\xabs{await g;s}) = \sem{\mathit{mte}(\xabs{g})}_\tau \\
\mathit{mte}(\tau,\mathit{fid},\xabs{s}) &= \infty\text{ if }\xabs{s}\neq \xabs{await g;s'}\qquad\qquad
\end{align*}
\end{minipage}} \vspace{2mm}

\noindent Note that \textit{mte} is not applied to
the currently active process, because, when \rulename{1} is not
applicable, it is currently blocking and, thus, cannot advance time.


The semantics trigger the guards as soon as possible. 
This is crucial for the simulation capabilities of \HABS. 
The more relaxed semantics of, e.g., hybrid automata, introduce additional non-determinism that is beneficial for verification but difficult to handle meaningfully for simulation.
We remind that we only allow weak inqualities, i.e., an event boundary always exists and the minimum indeed exists.

\paragraph{Runs}
The semantics of a programs are expressed as \emph{run}, generated by the operational semantics, and for each run a set of traces, one for each object. 

A trace $\theta$ is a mapping from $\mathbb{R}^+$ to states, meaning that at time $t$ the state of the program is $\theta(t)$.
A trace is extracted from a run by interpolating between two configurations resulting from discrete steps using the last solution.
We say that
$\mathsf{clock}(t_i)~\mathit{cn}_i$ is the final configuration at
$t_i$ in a run, if any other timed configuration
$\mathsf{clock}(t_i)~\mathit{cn}_i'$ is before it.
\begin{definition}[Traces]\label{def:trace}
Let \textsf{Prgm} be a program. Its initial state configuration is denoted $\mathsf{clock}(0)~\mathit{cn}_0$~\cite{BjorkBJST13}.
A run of \textsf{Prgm} is a
(possibly infinite) reduction sequence
\[\mathsf{clock}(0)~\mathit{cn}_0 \rightarrow \mathsf{clock}(t_1)~\mathit{cn}_1 \rightarrow \cdots\]
A run is \emph{time-convergent} if it is infinite and $\lim_{i \mapsto \infty} t_i < \infty$.
A run is \emph{locally terminated} if every process within terminates.
%The trace $\theta_o$ of an object $o$ in a run is an assignment from
%the dense time domain $\mathbb{R}^+$ to states.  

For each object $o$ occurring in the run, its \emph{trace} is defined as $\theta_o$ is 

\scalebox{0.9}{\begin{minipage}{\columnwidth}
\begin{align*}
\theta_o(x) = \cased{
\mathit{undefined} &\text{if $o$ is not created yet}\\
\rho &\text{if $\mathsf{clock}(x)~\mathit{cn}$ is the final configuration at $x$}\\ 
&\text{ and $\rho$ is the state of $o$ in $\mathit{cn}$.}\\
\mathit{adv}_{\mathit{heap}}(\rho,f,x-y) &\text{if there is no configuration at $\mathsf{clock}(x)$}\\
&\text{and the last configuration was at $\mathsf{clock}(y)$}\\
&\text{with state $\rho$ and dynamic $f$ }
}
\end{align*}
\end{minipage}}
\end{definition}
We normalize all traces and let them start with 0 by shifting all states by the time the object is created.

\begin{example}
Consider the following example, which illustrates the semantics of tank from Fig.~\ref{fig:bball}, starting at time 1:
\begin{align*}
&\mathsf{clock}(1)~\Big(o,\rho_1,\mathit{ODE},f,\bot,\big\{(\emptyset,\mathit{fid}_1,\statement^+_{\xabs{down}}),\mathit{prc}\big\}\Big)\\
\xrightarrow{(ii)}~&\mathsf{clock}(2)~\Big(o,\rho_2,\mathit{ODE},f,\bot,\big\{(\emptyset,\mathit{fid}_1,\statement^+_{\xabs{down}}),\mathit{prc}\big\}\Big)\\
\xrightarrow{(3)}~&\mathsf{clock}(2)~\Big(o,\rho_2,\mathit{ODE},f,(\emptyset,\mathit{fid}_1,\statement_{\xabs{down}}),\big\{\mathit{prc}\big\}\Big)\\
\xrightarrow{(7)}~&\mathsf{clock}(2)~\Big(o,\rho_2,\mathit{ODE},f,(\emptyset,\mathit{fid}_1,\dots),\big\{\mathit{prc}\big\}\Big)\quad\mathsf{msg}(o,\mathit{log},\mathit{fid}_2)
\end{align*}
The store is $\rho_1 = \{\xabs{level} \mapsto 4,\xabs{drain} \mapsto -1, \xabs{log} \mapsto \mathit{l}\}$ and two processes are suspended.
The one for \xabs{up} is denoted $\mathit{prc}$, the one for \xabs{down} has the remaining statement $\statement^+_{\xabs{down}}$, which is the whole method body.

Nothing can execute without advancing time, so time is advanced by 1 time unit (using rule (ii)) until the store changes to 
$\rho_1 = \{\xabs{level} \mapsto 3,\xabs{drain} \mapsto -1,\xabs{log} \mapsto \mathit{l}\}$.

This enables rule (3) to schedule the process for \xabs{down}, where the \abs{await} statement is removed: $\statement_{\xabs{down}}$ is the method body without the leading suspension.
Finally, rule (7) is used to generate a message to call the other object.
\end{example}








\paragraph{Methods and Transitions}
We stress that methods are more than just discrete transitions and are not necessarily instantaneous.
Consider, for example, the following the following code, which models two water tanks with a common valve.
The switch from filling one tank to another takes one time unit between the change of the first tank and the second one. Verification of methods, thus, must take concurrency \emph{and} time delays into account.

\noindent
\begin{minipage}{0.5\textwidth}
\begin{abscode}
class DoubleTank(){
    physical Real lvl1 = 5;
    physical Real lvl2 = 5;
    Real drain1 = 0.5;
    Real drain2 = -0.5;
    physical{ lvl1' = drain1;
             lvl2' = drain2; }
\end{abscode}
\end{minipage}
\begin{minipage}{0.5\textwidth}
\begin{abscode}

    Unit switch(){
        drain1 = -drain1;
        duration(1,1);
        drain2 = -drain2;
    }
}
\end{abscode}
\end{minipage}











\COMMENT{
A useful pattern, already applied in Ex.~\ref{ex:bball}, are controllers.
\begin{definition}[Controller]
A method is a \emph{controller} if it (1) starts with an \abs{await} (2) contains no other suspensions and neither \abs{get} nor \abs{duration} statements, (3) ends with a recursive call, (4) is called only from the initial block.
\end{definition}
Because of (2), a controller runs instantaneous and because of (3) and (4) always potentially schedulable. Analyzing the leading guard of (1) allows one to precisely see under which conditions it can be scheduled.

In Ex.~\ref{ex:bball} class \abs{Tank} is controlled by \abs{up} and \abs{down}.
Controllers are a natural modeling pattern: the largest Active Object case study (modeling railway operations~\cite{scp} in \texttt{ABS}) uses controllers for almost all active classes.

Semantics are defined as structural operational semantics, i.e., rewrite rules on runtime syntax. 
Runtime syntax represents the state of a program. The \HABS semantics are fairly standard, except that (1) we use the timed extension of Bj{\o}rk et al.~\cite{BjorkBJST13}, which allows
us to keep track of time in the semantics, and (2) that time advance changes not only the time, but also the object state, because it evolves according to the \abs{physical} block.
}

==> obl.tex <==
For \abs{Controller}, the following obligations are generated:
\begin{align*}
    init,\\
    ctrl,\\
    stop
\end{align*}
For the main block the following obligation is generated:
\begin{align*}
    init
\end{align*}
Note that the mechanism to verify method contracts is integrated into the logic itself~\cite{DBLP:conf/tableaux/Kamburjan19}, not based on a flag, which is only required due to restrictions of \ddl.
